Forensicability of Deep Neural Network Inference Pipelines

We propose methods to infer properties of the execution environment of machine learning pipelines by tracing characteristic numerical deviations in observable outputs. Results from a series of proof-of-concept experiments obtained on local and cloud-hosted machines give rise to possible forensic applications, such as the identification of the hardware platform used to produce deep neural network predictions. Finally, we introduce boundary samples that amplify the numerical deviations in order to distinguish machines by their predicted label only.

==> floats/amd_extension_explanation.tex <==
\begin{tabular}{r l}
    \toprule
    \textbf{Extension}         & \textbf{Explanation}                                              \\
    \midrule
    MMX               & Predecessor of SSE2                                                        \\
    SSE               & SIMD vector operation extensions                                           \\
    AES               & AES specialty instructions                                                 \\
    AVX               & SSE with more width and support for three operands                         \\
    AVX 2             & Extension of AVX with more general purpose vectorization                   \\
    BMI 1/1+/2        & Bit manipulation instruction set                                           \\
    SHA               & Specialized SHA instructions                                               \\
    F16C              & Half precision floating point instructions                                 \\
    SMAP              & Protect user-space memory from accidental access from supervisor mode      \\
    SMEP              & Protect user-space memory from accidental instruction from supervisor mode \\
    AMD64             & AMD's 64 bit instruction set extension while maintaining x86 compatibility \\
    Precision Boost 2 & AMD dynamic overclocking                                                   \\
    SMT               & "Simultaneous Multithreading" on a single CPU core                         \\
    XFR2              & AMD eXtended Frequency Range                                               \\
    Pure Power        & Dynamic power optimization \\
    \bottomrule
\end{tabular}

==> floats/batch_adversarial_cifar10.tex <==
\begin{tabular}{c  r  r  r  c} % last c again to fix loop
    \toprule
    \textbf{CPU}                & i & ii & iii & \\
    \midrule
    i            & 0.0     & 0.03               & 0.0          & \\
    ii & 0.03    & 0.0                & 0.03         & \\
    iii       & 0.0     & 0.03               & 0.0          & \\
    \bottomrule
\end{tabular}

==> floats/batch_adversarial_fmnist.tex <==
\begin{tabular}{c  r  r  r  c} % last c again to fix loop
    \toprule
    \textbf{CPU}                & i & ii & iii & \\
    \midrule
    i            & 0.0     & 0.12               & 0.0          & \\
    ii & 0.12    & 0.0                & 0.12         & \\
    iii       & 0.0     & 0.12               & 0.0          & \\
    \bottomrule
\end{tabular}

==> floats/batch_adversarial_mnist.tex <==
\begin{tabular}{c  r  r  r  c} % last c again to fix loop
	\toprule
    \textbf{CPU}                & i & ii & iii & \\
    \midrule
    i            & 0.0     & 0.48               & 0.0          & \\
    ii & 0.48    & 0.0                & 0.48         & \\
    iii       & 0.0     & 0.48               & 0.0          & \\
    \bottomrule
\end{tabular}

==> floats/extensions.tex <==
\begin{tabular}{r l}
	\toprule
    \textbf{CPU}                & \textbf{Extensions}                                                                                                                          \\
    \midrule                                                                                                                                                 \\
    Threadripper 2950X & \parbox{5cm}{MMX, SSE1-4.2, AES, AVX, AVX2, BMI, BMI1+ BMI2, SHA, F16C, SMAP, AMD64, SMEP, Precision Boost2, SMT, XFR2, Pure Power} \\
    i7-9700            & Intel® SSE4.1, Intel® SSE4.2, Intel® AVX2                                                                                           \\
    Xeon CPU E3-1270   & Intel® SSE4.1, Intel® SSE4.2, Intel® AVX2                                                                                           \\
    \bottomrule
\end{tabular}

==> floats/input_complexity-diagonal.tex <==
\begin{tabular}{c rrrrrrrrr   c} % last column is to make the loop work
    \textbf{Model} &
                    \multicolumn{9}{c}{{\begin{tabular}[c]{@{}c@{}}two\_conv\\$1 \times 3 \times 3$\end{tabular}}} &
         \\
                    \cmidrule(lr){2-10}
            \textbf{TF version} &
                                    \multicolumn{9}{c}{2.3.0} &
                            \\
                                    \cmidrule(lr){2-10}
                        \textbf{\begin{tabular}[c]{@{}c@{}}Diagonal\\Period\end{tabular}} &
                                    1 &
                                    2 &
                                    3 &
                                    4 &
                                    5 &
                                    6 &
                                    14 &
                                    15 &
                                    28 &
                                            \\

    \midrule

            A & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\
            B & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\
            C & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\
            D & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\
            E & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &\\
            F & 1 & 0 & 1 & 2 & 2 & 2 & 2 & 2 & 2 &\\
            G & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\
            H & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &\\
            I & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\

\end{tabular}


==> floats/input_complexity-horizontal.tex <==
\begin{tabular}{c rrrrrrrrr   c} % last column is to make the loop work
    \textbf{Model} &
                    \multicolumn{9}{c}{{\begin{tabular}[c]{@{}c@{}}two\_conv\\$1 \times 3 \times 3$\end{tabular}}} &
         \\
                    \cmidrule(lr){2-10}
            \textbf{TF version} &
                                    \multicolumn{9}{c}{2.3.0} &
                            \\
                                    \cmidrule(lr){2-10}
                        \textbf{\begin{tabular}[c]{@{}c@{}}Horizontal\\Period\end{tabular}} &
                                    1 &
                                    2 &
                                    3 &
                                    4 &
                                    5 &
                                    6 &
                                    14 &
                                    15 &
                                    28 &
                                            \\

    \midrule

            A & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\
            B & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\
            C & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\
            D & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\
            E & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &\\
            F & 1 & 0 & 2 & 2 & 2 & 2 & 2 & 2 & 2 &\\
            G & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\
            H & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &\\
            I & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\

\end{tabular}


==> floats/input_complexity-vertical.tex <==
\begin{tabular}{c rrrrrrrrr   c} % last column is to make the loop work
    \textbf{Model} &
                    \multicolumn{9}{c}{{\begin{tabular}[c]{@{}c@{}}two\_conv\\$1 \times 3 \times 3$\end{tabular}}} &
         \\
                    \cmidrule(lr){2-10}
            \textbf{TF version} &
                                    \multicolumn{9}{c}{2.3.0} &
                            \\
                                    \cmidrule(lr){2-10}
                        \textbf{\begin{tabular}[c]{@{}c@{}}Vertical\\Period\end{tabular}} &
                                    1 &
                                    2 &
                                    3 &
                                    4 &
                                    5 &
                                    6 &
                                    14 &
                                    15 &
                                    28 &
                                            \\

    \midrule

            A & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\
            B & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\
            C & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\
            D & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\
            E & 0 & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &\\
            F & 1 & 0 & 2 & 2 & 2 & 2 & 2 & 2 & 2 &\\
            G & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\
            H & 0 & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 &\\
            I & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &\\


\end{tabular}


==> floats/single_adversarial_cifar10.tex <==
\begin{tabular}{c@{~}c@{~}r@{~}r@{~}r}
    Architecture & Label & Confidence & 2. Conf.  & Difference \\
    \midrule
    Arch i       & 3     & 0.29437256 & 0.2943725 & 5.96e-08   \\
    Arch ii      & 3     & 0.29437256 & 0.2943725 & 5.96e-08   \\
    Arch iii     & 5     & 0.2943726  & 0.2943721 & 4.76e-07   \\
\end{tabular}

==> floats/single_adversarial_fmnist.tex <==
\begin{tabular}{c@{~}c@{~}r@{~}r@{~}r}
    Architecture & Label & Confidence & 2. Conf.   & Difference \\
    \midrule
    Arch i       & 4     & 0.31779698 & 0.31779516 & 1.81e-06   \\
    Arch ii      & 4     & 0.31779698 & 0.31779516 & 1.81e-06   \\
    Arch iii     & 0     & 0.31779578 & 0.31779578 & 0.0        \\
\end{tabular}

==> floats/single_adversarial_mnist.tex <==
\begin{tabular}{c@{~}c@{~}r@{~}r@{~}r}
    Architecture & Label & Confidence & 2. Conf.   & Difference    \\
    \midrule
    Arch i       & 9     & 0.49980018 & 0.49979922 & 9.53e-07      \\
    Arch ii      & 9     & 0.49980018 & 0.49979922 & 9.53e-07      \\
    Arch iii     & 4     & 0.49979982 & 0.49979958 & 2.38e-07 \\
\end{tabular}
